Benchmarking global optimization techniques for unmanned aerial vehicle path planning

The Unmanned Aerial Vehicle (UAV) path planning problem is a complex optimization problem in the field of robotics. In this paper, we investigate the possible utilization of this problem in benchmarking global optimization methods. We devise a problem instance generator and pick 56 representative instances, which we compare to established benchmarking suits through Exploratory Landscape Analysis to show their uniqueness. For the computational comparison, we select twelve well-performing global optimization techniques from both subfields of stochastic algorithms (evolutionary computation methods) and deterministic algorithms (Dividing RECTangles, or DIRECT-type methods). The experiments were conducted in settings with varying dimensionality and computational budgets. The results were analyzed through several criteria (number of best-found solutions, mean relative error, Friedman ranks) and utilized established statistical tests. The best-ranking methods for the UAV problems were almost universally the top-performing evolutionary techniques from recent competitions on numerical optimization at the Institute of Electrical and Electronics Engineers Congress on Evolutionary Computation. Lastly, we discussed the variable dimension characteristics of the studied UAV problems that remain still largely under-investigated.

==> history.tex <==
Since I am practising and making many mistakes, I will keep a hsitory of the text how it evolved over time 


08/03/2024

% Ali part
{\color{red} read from here}
\newline
The numerical results of different computational budgets, $1e3$ to $1e5$, are presented in tables \ref{tab-fe3},\ref{tab-fe4},\ref{tab-fe5}. Here the methods are compared in terms of three statistical perspectives. The first column displays the average relative error, which indicates how robust each method is, the lower the error, the more robust the method. the second column has a record of the number of wins, that is how many times had a certain method found the best solution among all others in the same terrain. This is a metric one would consider to evaluate which method has the most optimized path found. Lastly, the third column shows the Friedman rank. Since we have fifty-six different scenarios to compare over twelve algorithms, we opted to run the Friedman test which is suitable to detect differences in treatments across multiple test attempts. A lower Friedman rank indicates a method's superior performance. Therefore, the best three methods are highlighted in each table.

Moreover, the best method according to Friedman rank is denoted in tables \ref{tab-pe3},\ref{tab-pe4},\ref{tab-pe5} as 'best', and  a significance test, as well as an improved significance test, are conducted to determine how similar other method are in comparison to the best one. (could you add more test here on how the significance test were done)
% old Ali

% We Have conducted numerical experiments with different computational budgets, so let us start by examining the cheapest computation budget of E3
Analyzing the results collectively, it is clear that there is no monotony in the result and no single optimization method stands out as the clear winner for solving such problems. Rather, each setting of the problem would yield a better candidate than another. For instance, when considering a low computational budget $n_{max}=3$, we can observe in Table \ref{tab-fe3} Fig. \ref{fig:res1e3} that EA4eig is the best method for low-time, low budgets UAVs, attaining the lowest Friedman rank and the most number of wins over all decision variables. That is even bolstered by its robustness, as evidenced by its lowest average relative error in almost all cases, except in $DV=5$. Second best methods for low computation budgets are limited to APGSK, LSHADE \ref{tab-pe3}.

In the case that the UAV has an adequate computational budget $n_{max}=4,5$, two distinct perspectives can be sought after:
\begin{enumerate}
    \item Finding a method that is more likely to find the absolute shortest path. 
    \item Choosing a method that consistently yields paths close to the optimal ones. 
\end{enumerate}

The first criterion is dependant on the number of wins. In this regard, EA4eig excels, particularly in $DV=5$, while ELSHADE and APGSK demonstrate superior performance in $DV=10,15,20$. 
In terms of Robustness, APGSK consistently exhibits the lowest average relative error, making it the most robust option across all computational budgets. For $E4$, the top following robust methods predominantly include EA4eig and AGSK \ref{tab-fe4}. Similarly, for $E5$, the top three methods with the lowest relative error align closely with the lowest three Friedman ranks \ref{tab-fe5}.

Regarding Friedman ranks, although EA4eig outperforms ELSHADE in E3 and has a notable improvement given a larger budget, surpassing ELSHADE, \ref{perdev}. ELSHADE still finds more optimal paths in $DV =10,15$ and ranks better according to Friedman ranks \ref{tab-fe4}.
Nevertheless, even for larger search spaces, the difference is minimal \ref{tab-pe4}, and EA4eig maintains a low relative error, allowing it to surpass the null hypothesis of being similar to the best method in most cases.
 

APGSK and NM benefit the most from the higher allocated budget.
Analyzing the convergence plots of NM reveals that it finds non-optimal paths of high-costs in E3 , often crossing multiple threat areas, then it settles for "better" paths. While These paths are still far from being the optimal ones, a significant improvement over E4 and E5 must be admitted which is evident in \ref{perdev}.

On the contrary to NM, APGSK starts with paths that are closer to optimal ones \ref{tab-pe3}. Therefore, the enormous improvement demonstrated by APGSK, \ref{perdev}, makes it the top method of choice for E5 \ref{fig:conv}.






{\color{yellow} Till here}

